Rigorous asymptotic and moment-preserving diffusion approximations for generalized linear Boltzmann transport in arbitrary dimension

We derive new diffusion solutions to the monoenergetic generalized linear Boltzmann transport equation (GLBE) for the stationary collision density and scalar flux about an isotropic point source in an infinite $d$-dimensional absorbing medium with isotropic scattering. We consider both classical transport theory with exponentially-distributed free paths in arbitrary dimensions as well as a number of non-classical transport theories (non-exponential random flights) that describe a broader class of transport processes within partially-correlated random media. New rigorous asymptotic diffusion approximations are derived where possible. We also generalize Grosjean's moment-preserving approach of separating the first (or uncollided) distribution from the collided portion and approximating only the latter using diffusion. We find that for any spatial dimension and for many free-path distributions Grosjean's approach produces compact, analytic approximations that are, overall, more accurate for high absorption and for small source-detector separations than either $P_1$ diffusion or rigorous asymptotic diffusion. These diffusion-based approximations are exact in the first two even spatial moments, which we derive explicitly for various non-classical transport types. We also discuss connections between the random-flight-theory derivation of the Green's function and the discrete spectrum of the transport operator and report some new observations regarding the discrete eigenvalues of the transport operator for general dimensions and free-path distributions.

==> weibull.tex <==
\section{Weibull Random Flights}

  Here we consider non-classical transport with a Weibull free path distribution with unit mean and parameter $k > 0$,
    \begin{equation}
      p(s) = \frac{2^k k e^{-2^k \left(s \Gamma \left(k+\frac{1}{k}\right)\right)^k} \left(s
   \Gamma \left(k+\frac{1}{k}\right)\right)^k}{s}.
    \end{equation}
    When $k = 1$ the result is the exponential distribution.  Examples include
    \begin{equation}
      \left\{\frac{e^{-s/2}}{\sqrt{2 \pi } \sqrt{s}},e^{-s},4 e^{-2 s} s,\frac{27}{2}
   e^{-3 s} s^2,\frac{128}{3} e^{-4 s} s^3\right\} \in p(s),
    \end{equation}
    the second example with $k = 1$ being the exponential distribution.  The extinction function for Gamma flights is
    \begin{equation}
      E(s) = \frac{\Gamma (k,k s)}{\Gamma (k)}
    \end{equation}
    the mean square free path is
    \begin{equation}
      \langle s^2 \rangle = \frac{1}{k}+1
    \end{equation}
    and the mean square extinction is
    \begin{equation}
      \int_0^\infty E(s) s^2 = \frac{(k+1) (k+2)}{3 k^2}.
    \end{equation}
    In addition to recent time-resolved Gamma-flight solutions~\cite{caer11,pogorui11,pogorui13} we consider the steady-state collision densities of all orders, as well as the scalar flux, and diffusion approximations to both.

  \subsection{Gamma Random Flights---Rod Model ($d = 1$)}
    \subsubsection{Rod Model - Gamma $k = 1/2$}
      For $k = 1/2$, the transformed propagator in the rod is
      \begin{equation}
        \o{\zeta_1}(z) = \frac{\sqrt{z} \sqrt{\frac{\sqrt{4 z^2+1}+1}{4 z^3+z}}}{\sqrt{2}}.
      \end{equation}
      The characteristic equation yields two positive discrete eigenvalues,
      \begin{equation}
        \nu_0 = \frac{\sqrt{\frac{4
   c^2}{c^2-1}-\frac{8}{c^2-1}+\frac{c^4}{c^2-1} \pm \frac{\sqrt{c^2+8}
   c^3}{c^2-1}}}{\sqrt{2}}.
      \end{equation}
      The 2nd collision density can be found explicitly,
      \begin{equation}
        \Cpt(r|2) = \frac{c e^{-r/2} \left(2 e^{r/2} K_0\left(\frac{r}{2}\right)+\pi \right)}{8 \pi}, 
      \end{equation}
      as well as the 4th,
      \begin{equation}
        \Cpt(r|4) = \frac{c^3 \left(\pi  e^{-r/2} (r+6)+8 r K_1\left(\frac{r}{2}\right)\right)}{64\pi }. 
      \end{equation}

    \subsubsection{Rod Model - Gamma $k = 2$}
      For $k = 2$, the transformed Gamma propagator in the rod is
      \begin{equation}
        \o{\zeta_1}(z) = -\frac{4 \left(z^2-4\right)}{\left(z^2+4\right)^2}.
      \end{equation}
      The low order collision densities can be solved for explicitly,
      \begin{align}
        &\Cpt(r|2) = \frac{1}{12} c e^{-2 r} \left(8 r^3+6 r+3\right) \\
        &\Cpt(r|3) = \frac{1}{240} c^2 e^{-2 r} \left(2 r \left(r \left(8 r^3+30
   r+45\right)+45\right)+45\right)
      \end{align}
      Similar to classical transport in the rod, the rigorous collision-density diffusion solution is the exact solution in the rod, but with \emph{two} discrete diffusion terms
      \begin{equation}
        \Cpt(r) = \sum_{\chi} -\frac{\left(\chi ^4-16\right) e^{-r \chi }}{2 c \chi  \left(\chi ^2+12\right)}.
      \end{equation}
      The pair of positive discrete inverse diffusion lengths are
      \begin{equation}
        \chi \in \sqrt{2} \sqrt{2 + c \pm \sqrt{c (c+8)}}.
      \end{equation}

  \subsection{Gamma Random Flights---Flatland ($d = 2$)}
    \subsubsection{Flatland - Gamma $k = 2$}
      For $k = 2$, the transformed Gamma propagator in flatland is
      \begin{equation}
        \o{\zeta_2}(z) = \frac{8}{\left(z^2+4\right)^{3/2}}.
      \end{equation}
      The characteristic equation yields the single positive eigenvalue
      \begin{equation}
        \nu_0 = \frac{1}{2 \sqrt{1-c^{2/3}}}.
      \end{equation}
      The $n$th collision densities can be found explicitly
      \begin{equation}
        \Cpt(r|n) = \frac{2 c^{n-1} r^{\frac{3 n}{2}-1} K_{1-\frac{3 n}{2}}(2 r)}{\pi  \Gamma \left(\frac{3
   n}{2}\right)}.
      \end{equation}
      The $n$th scalar fluxes / fluences can also be found explicitly
      \begin{multline}
        \phipt(r|n) = \frac{c^n r^{\frac{3 n}{2}-\frac{1}{2}}}{4 \Gamma \left(\frac{3
   (n+1)}{2}\right)} [ 2 r I_{-\frac{3}{2} (n-1)}(2 r)-6 n I_{\frac{1}{2} (1-3 n)}(2 r) \\
   + (3 n+1) I_{\frac{1}{2} (3 n-1)}(2 r)-2 r I_{\frac{1}{2} (3 n+1)}(2 r) ] \sec \left(\frac{3 \pi  n}{2}\right).
      \end{multline}

  \subsection{Gamma Random Flights---3D}
    \subsubsection{3D - Gamma $k = 2$}
      For $k = 2$, the transformed propagator in 3D is
      \begin{equation}
        \o{\zeta_2}(z) = \frac{4}{z^2+4}.
      \end{equation}
      The characteristic equation yields the single positive eigenvalue
      \begin{equation}
        \nu_0 = \frac{1}{2 \sqrt{1-c}}.
      \end{equation}
      The $n$th collision densities can be found explicitly
      \begin{equation}
        \Cpt(r|n) = \frac{2 (c r)^{n-1} K_{\frac{3}{2}-n}(2 r)}{\pi ^{3/2} \sqrt{r} \Gamma (n)}.
      \end{equation}
      The exact total collision density is also found to be
      \begin{equation}
        \Cpt(r) = \frac{e^{-2 \sqrt{1-c} r}}{\pi  r}.
      \end{equation}
      Thus, we see in 3D a random flight model with the same spectrum as classical transport in a rod (scaled by a factor of 2), and the exact total collision density is diffusion.  However, we were unable to invert the scalar flux / fluence analytically.

  \subsection{Gamma Random Flights---General Dimension}
    The transformed propagator in $d$ dimensions is
    \begin{equation}\label{eq:gammaprop}
      \zeta_d(z) = \F \{ p(r) / \Omega_d(r) \} = \, _2F_1\left(\frac{k}{2},\frac{k+1}{2};\frac{d}{2};-\frac{z^2}{k^2}\right)
    \end{equation}
    which for the first few integer dimensions gives
    \begin{equation*}
     \begin{array}{llll}
     d & \zeta_d(z), k=2 & \zeta_d(z),k = 3 & \zeta_d(z),k = 4 \\
 1 & -\frac{4 \left(z^2-4\right)}{\left(z^2+4\right)^2} & -\frac{243
   \left(z^2-3\right)}{\left(z^2+9\right)^3} & \frac{256 \left(z^4-96
   z^2+256\right)}{\left(z^2+16\right)^4} \\
 2 & \frac{8}{\left(z^2+4\right)^{3/2}} & -\frac{27 \left(z^2-18\right)}{2
   \left(z^2+9\right)^{5/2}} & -\frac{512 \left(3 z^2-32\right)}{\left(z^2+16\right)^{7/2}}
   \\
 3 & \frac{4}{z^2+4} & \frac{81}{\left(z^2+9\right)^2} & -\frac{256 \left(z^2-48\right)}{3
   \left(z^2+16\right)^3} \\
 4 & \frac{8-\frac{16}{\sqrt{z^2+4}}}{z^2} & \frac{27}{\left(z^2+9\right)^{3/2}} &
   \frac{1}{\left(\frac{z^2}{16}+1\right)^{5/2}} \\
 5 & \frac{12 \left(z-2 \tan ^{-1}\left(\frac{z}{2}\right)\right)}{z^3} & \frac{81
   \left(\left(z^2+9\right) \tan ^{-1}\left(\frac{z}{3}\right)-3 z\right)}{2 z^3
   \left(z^2+9\right)} & \frac{256}{\left(z^2+16\right)^2} \\
    \end{array}
    \end{equation*}

    For Gamma random flights in $d$ dimensions, the first few even collision density moments are
      \begin{align}
        &\int_0^\infty \Omega_d(r) \Cpt(r|n) dr = c^{n-1} \\
        &\int_0^\infty \Omega_d(r) r^2 \Cpt(r|n) dr = \frac{(k+1) n c^{n-1}}{k} \\
        &\int_0^\infty \Omega_d(r) r^4 \Cpt(r|n) dr = \\ &\frac{(k+1) n c^{n-1} (d (k (k n+n+4)+6)+2 k (k+1) (n-1))}{d k^3}
      \end{align}
      and the total collision density moments
      \begin{align}
        &\int_0^\infty \Omega_d(r) \Cpt(r) dr = \frac{1}{1-c} \\
        &\int_0^\infty \Omega_d(r) r^2 \Cpt(r) dr = \frac{k+1}{(c-1)^2 k} \\
        &\int_0^\infty \Omega_d(r) r^4 \Cpt(r) dr = \\ &-\frac{(k+1) (d (c ((k-3) k-6)+(k+2) (k+3))+4 c k (k+1))}{(c-1)^3 d k^3}.
      \end{align}

      The first few even $n$th scattered scalar flux / fluence moments are
      \begin{align}
        &\int_0^\infty \Omega_d(r) \phipt(r|n) dr = c^n \\
        &\int_0^\infty \Omega_d(r) r^2 \phipt(r|n) dr = \frac{(k+1) c^n (3 k n+k+2)}{3 k^2}
      \end{align}
      and the total scalar flux / fluence moments are
      \begin{align}
        &\int_0^\infty \Omega_d(r) \phipt(r) dr = \frac{1}{1-c} \\
        &\int_0^\infty \Omega_d(r) r^2 \phipt(r) dr = \frac{(k+1) (2 c (k-1)+k+2)}{3 (c-1)^2 k^2}.
      \end{align}
      Again, we see that the first two even moments are dimension independent.

    \subsubsection{Gamma Flights Collision Density Diffusion}
      The Pade approximant producing the transformed classical $P_1$ diffusion approximation for the total collision density is
      \begin{equation}
        \frac{\o{\zeta}_d(z)}{1 - \ssalbedo \o{\zeta}_d(z)} \approx -\frac{2 d k}{2 (c-1) d k-(k+2) z^2}
      \end{equation}
      yielding the collision density $P_1$ diffusion length
      \begin{equation}
        \nu_0^2 = \frac{k+2}{2 d k-2 c d k}.
      \end{equation}
      Likewise, the Grosjean collision density diffusion length is given by
      \begin{equation}
        \nu_G^2 = \frac{(c-2) (k+1)}{2 (c-1) d k}.
      \end{equation}

    \subsubsection{Gamma Flights Scalar Flux Diffusion}
      The transformed stretched extinction propagator is
      \begin{equation}
        \o{X(z)} = \, _3F_2\left(\frac{1}{2},\frac{k}{4}+\frac{1}{2},\frac{k}{4}+1;\frac{3}{2},\frac{d}{2};-\frac{4 z^2}{k^2}\right)
      \end{equation}
      where $_3F_2$ is a hypergeometric function.  This yields the scalar flux diffusion length
      \begin{equation}
        \nu_0^2 = \frac{(-k-1) (2 c (k-1)+k+2)}{6 (c-1) d k^2}
      \end{equation}
      where agrees with the classical exponential result when $k = 2$.  The Grosjean diffusion length for the scalar flux / fluence is
      \begin{equation}
        \nu_G^2 = \frac{(k+1) (c (k+2)-4 k-2)}{6 (c-1) d k^2}.
      \end{equation}
       

